Activity Report on the Eighth African School of Fundamental Physics and Applications (ASP2024)

The African School of Fundamental Physics and Applications, also known as the African School of Physics (ASP), was initiated in 2010, as a three-week biennial event, to offer additional training in fundamental and applied physics to African students with a minimum of three-year university education. Since its inception, ASP has grown to be much more than a school. ASP has become a series of activities and events to support academic development of African students, teachers and faculties. We report on the eighth African School of Physics, ASP2024, organized in Morocco, on April 15--19 and July 7--21, 2024. ASP2024 included programs for university students, high school teachers and high school pupils.

==> expenseTable.tex <==
The total expenditures amounts to \texteuro197499 as shown in Table~\ref{tab:table2}; that leaves a surplus of \texteuro5586.
\begin{table}[!htbp]
\centering
\begin{tabular}{l|r}
\hline\hline
\textbf{Item}    &  \textbf{Cost} \\ \hline
ICTP Travel coverage for African students \& lecturers & 32000 \\
Other travels, room and board, equipment, logistics & 112499\\
ASP2024 student oral presentation awards& 3000\\
Unused because of entrance visa problems & 10000 \\
Earmarked for ACP2025  & 40000\\
 \hline\hline
\end{tabular}
\caption{Expenditures for ASP2024 (and expected for ACP2025) in Euros. The ICTP support was used at the ICTP to cover travel for selected African students, materials and invited lecturers associated to the ICTP 60th anniversary celebration~\cite{ICTP-ASP2024}. The other contributions received were used to cover transportation, room \& board, equipment and logistics for high school, teachers and students programs; SAIP collected and aggregated the contributions and handled all payments in these categories. We reserved \texteuro3000 for 3 student best oral presentations---we received 23 abstracts from ASP2024 participants. At the time of writing, the abstracts were under reviews by a committee of ASP lecturers and the oral presentations of selected abstracts scheduled in October 2024. Finally, 20\% of the support received (in this case \texteuro40000) were earmarked towards coverage for ACP2025 mentioned in Section~\ref{sec:out}. Some selected participants could not travel because of visa application problems and about \texteuro10000 were not spent as a result---these funds will be used towards future ASP events. The small surplus of \texteuro5586 was due to the fact the organizing committee (local and international) made efforts to optimize expenditures without compromising the quality of the services rendered.}
\label{tab:table2}
\end{table}



==> supportTable.tex <==
The summed contributions received, shown in Table~\ref{tab:table1}, amounted to about \texteuro203085.
\begin{table}[!htbp]
\centering
\begin{tabular}{l|r|l}
\hline\hline
\textbf{Source}    &  \textbf{Amount} & \textbf{Currency} \\ \hline
DOE (USA)           &   43495  & Dollar     \\
ICTP (Italy)              & 32000 & Euro\\
STCF / IOP (UK)     & 30000 & Euro \\
INFN (Italy)              & 15000 & Euro\\
NSF  (USA)              & 14000 & Dollar \\
SUNY Old Westbury       & 12460 & Dollar \\
Argonne National Laboratory & 10000 & Dollar \\
IUPAP                   & 7000 & Euro \\
University of Birmingham (UK) & 5000 & GBP \\
Lee Foundation (Taiwan) & 6000 & Euro \\
GSSI (Italy)  & 5000 & Euro \\
IFAE (Spain)  & 5000 & Euro \\
CERN (Switzerland) & 5000 & CHF \\
FNAL (USA)         & 5000 & Dollar \\
APS (USA) & 5000 & Dollar \\
PSI (Switzerland)  & 4000 & CHF \\
DESY (Germany)  & 3000 & Euro \\
NITheCS (South Africa) & 100000 & Rand \\
Dr. Joseph Mitchell (USA) & 3500 & Dollar \\
ESS (Sweden)  & 3000 & Euros \\
MacDonald Institute (Canada) & 1000 & Canadian Dollar \\
 \hline\hline
\end{tabular}
\caption{Contributions to the ASP2024 and ACP2025 budget.}
\label{tab:table1}
\end{table}


